Causal-ICM: A Data Fusion Framework For Heterogeneous Treatment Effect Estimation With Multi-Task Gaussian Processes

Bridging the gap between internal and external validity is crucial for heterogeneous treatment effect estimation. Randomised controlled trials (RCTs), favoured for their internal validity due to randomisation, often encounter challenges in generalising findings due to strict eligibility criteria. Observational studies, on the other hand, may provide stronger external validity through larger and more representative samples but can suffer from compromised internal validity due to unmeasured confounding. Motivated by these complementary characteristics, we propose a novel Bayesian nonparametric approach, Causal-ICM, leveraging multi-task Gaussian processes to integrate data from both RCTs and observational studies. In particular, we introduce a parameter that controls the degree of borrowing between the datasets and prevents the observational dataset from dominating the estimation. We propose a data-adaptive procedure for choosing the optimal value of the parameter. Causal-ICM outperforms other data fusion methods in point estimation across the covariate support of the observational study and provides principled uncertainty quantification for the estimated treatment effects. We demonstrate the robust performance of Causal-ICM in diverse scenarios through multiple simulation studies and a real-world study.

==> introduction.tex <==
\section{Introduction}

Treatment effect estimation is an important task in many applications, including medicine, epidemiology, and the social sciences. The goal is to quantify the expected impact of a particular intervention in a given target population. For instance, in medicine, one may seek to estimate the expected benefit or harm from taking a particular drug relative to placebo for a patient with a certain disease. 

%The \gls{ate} from a study is often used as evidence for whether a particular intervention should be applied to an individual or unit in a given target population. The reliability of this evidence rests on two key assumptions. Firstly, the study population is assumed to be sufficiently similar to the target population, so that an estimate of the treatment effect is applicable to the target population in which the intervention under investigation will eventually be applied. Secondly, the average treatment effect is assumed to be close to an individual's treatment effect.  

%This second assumption of homogeneity across individuals is often violated: 
The effect of an intervention within a population may vary systematically with respect to a particular set of covariates. Returning to the medical example, the effect of a drug may vary with a patient's age or sex. Understanding such treatment effect heterogeneity is critical to ensure that appropriate decisions are taken for all individuals, not just those similar to the average \citep{brantner_methods_2023}. 

%Whether the results of a study are relied upon for a particular decision or policy also depends on the statistical significance of the corresponding estimates. 
%A proposed intervention with an estimated positive treatment effect may not be adopted if statistical variability indicates that this estimate is not significantly away from zero. 
An appropriate characterisation of the uncertainty of treatment effect estimates is also required to support robust and reliable decision-making. 
%While this is reasonably straightforward in the computation of average treatment effects, 
Uncertainty quantification for heterogeneous treatment effects is challenging, however, especially when making inferences about individuals not represented in the study. Classical methods typically rely heavily on extrapolation without adequate variance inflation outside the study support \citep{degitar_review}.

The gold standard for treatment effect estimation remains the \glsfirst{rct}. The random treatment allocation in the study guards against the effect of confounding, assuming perfect compliance with the allocated treatment. As a result, under a few additional assumptions, the difference in average outcomes between individuals in the treatment and control arms is unbiased for the average treatment effect in the study population.

There are, however, drawbacks to the use of \glspl{rct} \citep{frieden2017}. They are typically expensive to carry out, and sample sizes can be limited as a result. While they may be powered enough to detect the main effect, they are typically underpowered for subgroup effects. Further, the study population may not be representative of the target population. This can be for a variety of reasons such as inclusion/exclusion criteria of individuals into the study (either on statistical, practical, or ethical grounds), or selection bias of individuals into the study; for instance, there may be differential acceptance to ``invitation to participate" from eligible candidates according to, for example, socioeconomic status, educational levels or ethnicity \citep{nas2022}.

Observational, or `real-world' studies, provide an alternative source of data for treatment effect estimation. In contrast to \glspl{rct}, they generally benefit from larger sample sizes and tend to be more representative of the target population. On the other hand, observational studies may suffer from unmeasured confounding. This occurs due to hidden variables that affect both the outcome of interest and the treatment allocation, and can lead to biased treatment effect estimates.

%a number of assumptions must be made to ensure the validity of treatment effect estimations from observational data. In particular, one must assume that there are no unmeasured confounders - hidden variables that affect both the outcome of interest and the treatment allocation. While it may be possible to adjust for the effect of observed confounders, there is no way to mitigate the effect of unmeasured confounding without making strong assumptions about the nature of confounding. 

The complementary nature of \gls{rct} and observational data indicates the potential benefits from combining the two sources to obtain better heterogeneous treatment effect estimates. Such data fusion approaches have received increased interest in recent years. A range of methods have been developed to integrate information from multiple sources of data, including a limited number targeting causal inference problems (see \cite{colnet_causal_2023} for a recent review). %To our knowledge, none of these approaches have leveraged the Bayesian non-parametric framework for extrapolation with uncertainty quantification, and most of them make strong untestable assumptions about the structure of the confounding effect.
These typically rely on strong, untestable assumptions about the structure of the confounding effect and, moreover, are not able to provide uncertainty quantification around the point estimates of heterogeneous treatment effects.

In this paper, we introduce a Bayesian nonparametric approach to obtain estimates, with uncertainty, of heterogeneous treatment effects for the target population. Our approach is based on a multi-output \gls{gp}. This a particularly natural choice in the data fusion context as it allows us to model the \gls{rct} and observational heterogeneous treatment effects as {correlated functions}, and use the Bayesian machinery to share information and quantify uncertainty of the functions in regions of differing covariate support.


Our key contributions are as follows:
\begin{itemize}
    \item We introduce an \gls{icm} for heteregeneous treatment effect estimation, which we call \textit{Causal-ICM}. \textit{Causal-ICM} is a multi-task \gls{gp} model that enables {accurate treatment effect estimation} within and outside of the support of the \gls{rct} and {principled uncertainty quantification} of treatment effect estimates across the support of the target population.
    %, without relying on strong assumptions on the structure of the hidden confounding effect.
    \item \textit{Causal-ICM} has a straightforward interpretation, relying on a key hyperparameter that quantifies the measure of trust in the quality of the observational data, and can be tuned data-adaptively. We provide theory to demonstrate that the \gls{icm} is robust against the dominating nature of a large observational dataset.
    \item We demonstrate excellent empirical performance in simulations and a real dataset relative to other causal data fusion methods for both point estimation and uncertainty quantification.
\end{itemize}


Our key contributions are as follows:
\begin{itemize}
    \item We propose \textit{Causal-ICM}, a multi-task \gls{gp} model for heterogeneous treatment effect estimation that accurately captures complex functional relationships in the presence of unobserved confounding both within the support of the \gls{rct} covariate distribution and when extrapolating beyond it.
    
    \item \textit{Causal-ICM} provides principled uncertainty quantification across the full support of the target population that is not dominated by the large sample size of the observational study.
    
    \item Through a comprehensive set of simulation studies and an application to a real-world dataset, we demonstrate that \textit{Causal-ICM} achieves similar or superior performance both in point estimation and uncertainty quantification relative to a broad set of state-of-the-art causal data fusion methods.
\end{itemize}






==> lit_review.tex <==
\section{Related Literature}

\Gls{hte} estimation has received renewed interest in recent years. The most common strategy is to focus on the \gls{cate} function, which quantifies the expected treatment effect given particular covariate values. Under suitable identifiability assumptions \citep{dahabreh_extending_2019}, the \gls{cate} can be estimated parametrically - e.g. using linear regression - or non-parametrically, e.g. using nearest-neighbour matching, kernel methods \citep{brantner_methods_2023}, or tree-based methods including causal random forests \citep{wager_estimation_2018} and their Bayesian counterpart \citep{hahn_bayesian_2020}.

% Data fusion for ATE
Data fusion across an \gls{rct} and an observational study builds on several lines of work. \cite{dahabreh_extending_2019} explored the generalisability of \gls{rct} inference to different target populations using g-methods (including reweighting methods) and doubly robust estimators. ADD REFERENCE TO XI LIN'S REVIEW. \cite{demirel2024predictionpoweredgeneralizationcausalinferences} propose a generalizability framework that builds an observational predictor and then treat the difference between the trial outcome function and that observational predictor as a bias function that captures both confounding and transportation bias due to the differences between the trial and target populations. Similar approaches, but outside the scope of our work, have focused on data fusion for the estimation of long term effects, where randomised data are unconfounded but contain only short term effects, while observational data, although confounded, contain information about long term outcomes (\cite{ghassami2025combiningexperimentalobservationaldata}, \cite{imbens2024longtermcausalinferencepersistent}). 

% Data fusion for CATE
 Others have used \gls{rct} data to correct for the possible (hidden) confounding effect present in observational data. For example, \cite{wu_integrative_2022} developed an R-learner and proved consistency and asymptotic efficiency of the estimator under the assumption of overlap between the \gls{rct} and observational study. \cite{kallus_removing_2018} employed a two-step approach to correct for hidden confounding in the absence of covariate overlap. Their approach relies on the strong assumption of linearity of the hidden confounding effect term (see Section~\ref{sec:fusion}) and hinges on achieving parametric identification of this correction term, ultimately yielding a consistent estimate of \gls{cate} over the confounded sample. In a related approach, \citet{yang_improved_2022} relaxed the linearity assumption and established identifiability and efficiency results under more general parametric structural models for the confounding effect. \citet{lin_many_2023} take yet another approach and use a power likelihood to reduce the effect of hidden confounding. \cite{hatt_combining_2022} propose a representation-learning approach that learns shared features and confounded outcome models from observational data, then uses the \gls{rct} to estimate a bias function that debiases these models, with finite-sample bounds characterizing how performance depends on sample size, distributional shift, and bias complexity.  \cite{Yang2023Elastic} propose a test-then-pool approach for combining \glspl{rct} and observational data for heterogeneous treatment effect estimation, pooling the datasets only when no bias is detected, though the method is limited to linear treatment effect models and relies on strong parametric assumptions. 

Our method, \textit{Causal-ICM}, employs multi-task \glspl{gp} (see \citet{alvarez_kernels_2012} for a review) to combine information from distinct studies for the purpose of \gls{cate} estimation. This builds on work that leverages multi-task \glspl{gp} for solely observational data, whereby each potential outcome is treated as a distinct task \citep{alaa_bayesian_2017}. GP-SLC is a similar approach that is able to handle hierarchical hidden confounders \citep{witty2020}. Others have built on this framework to develop a general class of counterfactual multi-task deep kernel models that efficiently estimate causal effects and learn policies by stacking coregionalized Gaussian Processes and Deep Kernels \citep{caron_counterfactual_2022}. \glspl{gp} have also been employed as a matching tool for causal inference \citep{huang2023}.



==> lit_review2.tex <==
\section{Related Literature}

\Gls{hte} estimation has received renewed interest in recent years. The most common strategy is to focus on the \gls{cate} function, which quantifies the expected treatment effect given particular covariate values. Under suitable identifiability assumptions \citep{dahabreh_extending_2019}, the \gls{cate} can be estimated parametrically - e.g. using linear regression - or non-parametrically, e.g. using nearest-neighbour matching, kernel methods \citep{brantner_methods_2023}, or tree-based methods including causal random forests \citep{wager_estimation_2018} and their Bayesian counterpart \citep{hahn_bayesian_2020}.

% Data fusion for ATE
Data fusion across an \gls{rct} and an observational study has tended to focus on \gls{ate} estimation (see \cite{lin2024datafusionefficiencygain} and \cite{colnet_causal_2023} for comprehensive reviews). These methods aim to improve efficiency by integrating information from both sources. \cite{demirel2024predictionpoweredgeneralizationcausalinferences} focus instead on data fusion for generalisability, proposing a framework that builds an observational predictor and then treat the difference between the trial outcome function and that observational predictor as a bias function that captures both confounding and transportation bias due to the differences between the trial and target populations. Similar approaches, although outside the immediate scope of our work, have focused on data fusion for the estimation of long term effects, where randomised data are unconfounded but contain only short term effects, while observational data, although confounded, contain information about long term outcomes (\cite{ghassami2025combiningexperimentalobservationaldata}, \cite{imbens2024longtermcausalinferencepersistent}). 

% Data fusion for CATE
Data fusion methods for \gls{cate} estimation, the focus of this paper, follow three broad lines of work. One strategy is to use experimental data to debias observational estimates by learning a correction or bias function. \cite{kallus_removing_2018} introduce a two-step approach that corrects hidden confounding in the absence of covariate overlap, relying on the strong assumption of linear confounding and the ability to identify this correction term parametrically. \citet{yang_improved_2022} relax this linearity assumption and provide identifiability and efficiency results under more flexible structural models. \cite{hatt_combining_2022} develop a representation-learning strategy that learns shared features and confounded outcome models from observational data, using the \gls{rct} to estimate a bias function that debiases these models, with finite-sample bounds that highlight how performance depends on sample size, distribution shift, and bias complexity. \cite{wu_integrative_2022} propose an R-learner that achieves consistency and asymptotic efficiency under covariate overlap between the \gls{rct} and the observational study. A second direction consists of ``test-then-pool'' strategies, in which the trial and observational datasets are combined only if the observational study appears sufficiently unbiased. For instance, \cite{Yang2023Elastic} implement such a strategy, although their approach is limited to linear treatment effect models and relies on strong parametric assumptions. A third line of work uses Bayesian dynamic borrowing to regulate how much information is extracted from the observational study. For instance, \cite{lin_many_2023} propose a Bayesian dynamic borrowing approach through a power likelihood to reduce the effect of confounding and control the degree of information we borrow from the observational study.

% Gaussian processes
Our method, \textit{Causal-ICM}, takes a Bayesian dynamic borrowing approach based on multi-task \glspl{gp}, whereby each potential outcome is treated as a distinct task. Multi-task \glspl{gp} have been successfully employed for causal inference using solely observational data \citep{alaa_bayesian_2017} and extended to handle hierarchical hidden confounders \citep{witty2020}. Others have built on this framework to develop a general class of counterfactual multi-task deep kernel models that efficiently estimate causal effects and learn policies by stacking coregionalized \glspl{gp} and deep kernels \citep{caron_counterfactual_2022}. \glspl{gp} have also been employed as a matching tool for causal inference \citep{huang2023}. However, these methods are limited to purely observational settings; here we extend these ideas by enabling inference in a data-fusion setting. Our approach is most similar to concurrent work employing multi-task \glspl{gp} for pseudo-outcome regression to obtain error bounds on the observational bias term \citep{fawkes2025}.

% ADD JAKE'S PAPER



